Optimal complexity solution of space-time finite element systems for state-based parabolic distributed optimal control problems

We consider a distributed optimal control problem subject to a parabolic evolution equation as constraint. The control will be considered in the energy norm of the anisotropic Sobolev space $[H_{0;,0}^{1,1/2}(Q)]^\ast$, such that the state equation of the partial differential equation defines an isomorphism onto $H^{1,1/2}_{0;0,}(Q)$. Thus, we can eliminate the control from the tracking type functional to be minimized, to derive the optimality system in order to determine the state. Since the appearing operator induces an equivalent norm in $H_{0;0,}^{1,1/2}(Q)$, we will replace it by a computable realization of the anisotropic Sobolev norm, using a modified Hilbert transformation. We are then able to link the cost or regularization parameter $\varrho>0$ to the distance of the state and the desired target, solely depending on the regularity of the target. For a conforming space-time finite element discretization, this behavior carries over to the discrete setting, leading to an optimal choice $\varrho = h_x^2$ of the regularization parameter $\varrho$ to the spatial finite element mesh size $h_x$. Using a space-time tensor product mesh, error estimates for the distance of the computable state to the desired target are derived. The main advantage of this new approach is, that applying sparse factorization techniques, a solver of optimal, i.e., almost linear, complexity is proposed and analyzed. The theoretical results are complemented by numerical examples, including discontinuous and less regular targets. Moreover, this approach can be applied also to optimal control problems subject to non-linear state equations.

==> includes/factorization_solver.tex <==
\subsection{Direct solver}
Writing down the system $K_h \vec{u} = \vec{f}$  again
\begin{align}
    \left(M_{h_t} \otimes M_{h_x} + \rho A_{h_t} \otimes M_{h_x} + \rho M_{h_t} \otimes K_{h_x}\right) \vec{u} = \vec{f},
\end{align}
we first multiply from the left by $M_{h_t}^{-1} \otimes I_{h_x}$ to obtain
\begin{align}
    \left(I_{h_t} \otimes M_{h_x} + \rho M_{h_t}^{-1}A^{H}_{h_t} \otimes M_{h_x} + \rho I_{h_t} \otimes K_{h_x}\right) \vec{u} = \left(M_{h_t}^{-1} \otimes I_{h_x}\right)\vec{f}. \label{eq:directsolver:firstStep}
\end{align}
Let $S_{h_t}$ be the matrix containing the eigenvectors of the matrix $M_{h_t}^{-1}A^{H}_{h_t}$ as columns and $\Lambda$ be the diagonal matrix containing the corresponding eigenvalues. These eigenvectors and values can be computed by solving the generalized eigenvalue problem
\begin{align}
    A_{h_t} \vec{v} = \lambda M_{h_t} \vec{v},
\end{align}
which is done analytically in Lemma \ref{lem:eigenvalues}.
Note that all eigenvalues are positive and real as $A_{h_t}$ as well as $M_{h_t}$ are symmetric and positive definite. Now we can bring the system into time-diagonal form by defining
\begin{align}
    \vec{u} = \left(S_{h_t} \otimes I_{h_x}\right) \vec{v}
\end{align}
and multiplying \eqref{eq:directsolver:firstStep} from the left by $S_{h_t}^{-1} \otimes I_{h_x}$ to obtain
\begin{align}
    \left(I_{h_t} \otimes M_{h_x} + \rho \Lambda \otimes M_{h_x} + \rho I_{h_t} \otimes K_{h_x}\right) \vec{v} = \left(S_{h_t}^{-1} M_{h_t}^{-1} \otimes I_{h_x}\right)\vec{f} = \vec{g}.
\end{align}
Now we can solve the system for each time step independently by solving the system
\begin{align}
    \left(M_{h_x} + \rho \lambda_i M_{h_x} + \rho K_{h_x}\right) \vec{v}^{(i)} = \vec{g}^{(i)} \label{eq:directsolver:spatialProblems}
\end{align}
where $\vec{v}^{(i)}$ and $\vec{g}^{(i)}$ are the $i$-th blocks of $\vec{v}$ and $\vec{g}$ with respect to the tensor product structure.
The spatial problems \eqref{eq:directsolver:spatialProblems} are all symmetric, positive definite and spectrally equivalent to the mass matrix $M_{h_x}$ which can be shown analogously to Lemma \ref{lem:spectralEquivalence}. As we use equally spaced grids, they are well suited for efficient solution by the conjugate gradient method, even without preconditioning.

Note that $M_{h_t}$ is of tridiagonal form and thus can be inverted efficiently with linear complexity. So the only two performance bottlenecks are the inversion of $S_{h_t}$ as well as the multiplication by $S_{h_t}$ as these are dense matrices. In summary, we end up with a complexity of $\mathcal{O}(N_t^2M_x)$. The term quadratic in $N_t$ comes from multiplications with $S_{h_t}$ and $S_{h_t}^{-1}$ which can be massively parallelized and are usually not a bottleneck due to the fact, that $N_t \ll M_x$ in most applications. However, when considering the case of a large number of time steps, e.g when parabolic scaling is needed or the time horizon is large, the quadratic effort is unpleasant. Taking a closer look on the matrix vector product
\begin{align}
    w_k = \left(S_{h_t} \vec{v}\right)_i = \sum_{l=0}^{N_t-1} \sin \left(\left(\frac{\pi}{2}+l \pi\right) \frac{i}{n}\right) v_l, \quad i = 1, \dots, N_t,
\end{align}
we notice, that it is two times the type two discrete sine transform of $\vec{v}$. The discrete sine transform as well as its inverse are closely related to the discrete Fourier transform, well understood and can be computed efficiently with $\mathcal{O}(N_t \log N_t)$ complexity \cite{FFTW05}. This is the approach we use in our implementation.
